Cybercrime Bitcoin Revenue Estimations: Quantifying the Impact of Methodology and Coverage

Multiple works have leveraged the public Bitcoin ledger to estimate the revenue cybercriminals obtain from their victims. Estimations focusing on the same target often do not agree, due to the use of different methodologies, seed addresses, and time periods. These factors make it challenging to understand the impact of their methodological differences. Furthermore, they underestimate the revenue due to the (lack of) coverage on the target's payment addresses, but how large this impact remains unknown. In this work, we perform the first systematic analysis on the estimation of cybercrime bitcoin revenue. We implement a tool that can replicate the different estimation methodologies. Using our tool we can quantify, in a controlled setting, the impact of the different methodology steps. In contrast to what is widely believed, we show that the revenue is not always underestimated. There exist methodologies that can introduce huge overestimation. We collect 30,424 payment addresses and use them to compare the financial impact of 6 cybercrimes (ransomware, clippers, sextortion, Ponzi schemes, giveaway scams, exchange scams) and of 141 cybercriminal groups. We observe that the popular multi-input clustering fails to discover addresses for 40% of groups. We quantify, for the first time, the impact of the (lack of) coverage on the estimation. For this, we propose two techniques to achieve high coverage, possibly nearly complete, on the DeadBolt server ransomware. Our expanded coverage enables estimating DeadBolt's revenue at $2.47M, 39 times higher than the estimation using two popular Internet scan engines.

==> Makefile <==
PROJECT=paper

# xfig documents whose corresponding EPS fies are used in the paper
# FIGFILES = segment.fig allocGroup.fig

# matlab scripts that generate output for the paper. These are *.m files
# that generate a corresponding *.eps file when run.
MFILES =

# GNUplot files
PLTFILES = 

# Other EPS files that are necessary to build the document
# If you have eps files that you generate by hand, list them here.
EPSFILES =

# Non-refdbms bib files to be included
# If you need a local .bib file, put that here.
LOCALBIB = bibliography/paper.bib
LOCALXTXBIB = bibliography/paper.xtx

# default targets to make for make all
TARGETS = $(PROJECT).pdf
TARGETSPS = $(PROJECT).ps

#-- Programs used when runing latex etc.                       
BIBTEX = bibtex
XTEX = crosstex
LATEX = latex
DVIPS = dvips -tletter
FIG2DEV = fig2dev
MATLAB = matlab
GNUPLOT = gnuplot
PS2PDF = ps2pdf
PDFLATEX = pdflatex

SRCFILES = $(wildcard *.tex tbl/*.tex)
EPSFIGFILES = $(FIGFILES:.fig=.eps)
EPSMFILES = $(MFILES:.m=.eps)
EPSPLTFILES = $(PLTFILES:.plt=.eps)
EPSFILES += $(EPSFIGFILES) $(EPSMFILES) $(EPSPLTFILES)

#--------------------------------------------------------------------------
# Production/target rules                       
#--------------------------------------------------------------------------
.SUFFIXES:
.PHONY: clean all veryclean
#-- EPS files may be expensive to regenerate, so keep them even though they
#-- are intermediate targets
.PRECIOUS: $(EPSMFILES) $(EPSFIGFILES)
#.PRECIOUS: $(EPSMFILES)

all: $(TARGETS)

#-- Make EPS files from matlab documents
%.eps: %.m
	$(MATLAB) -nodesktop -r "$*;quit" || $(MATLAB) -nodisplay -r "$*;quit"

#-- Make EPS files from xfig documents
%.eps: %.fig
	$(FIG2DEV) -L eps $< $@ || $(FIG2DEV) -L ps $< $@

#-- Make EPS files from GNUplot scripts
%.eps: %.plt
	$(GNUPLOT) $<

#-- Creation of initial .aux file
%.aux: %.tex $(SRCFILES) $(EPSFILES)
	$(LATEX) $<

#-- Create .bbl from .bib
%.bbl: %.aux $(LOCALBIB)
	$(BIBTEX) $*
	$(LATEX) $*.tex
	$(LATEX) $*.tex

#-- Build a dvi... 
#%.dvi: %.tex %.bbl $(EPSFILES) $(LOCALBIB)
%.dvi: %.tex %.bbl
	$(LATEX) $<

#-- converting .dvi to .ps... requires the EPS files
%.ps: %.dvi $(EPSFILES)
	$(DVIPS) -o $@ $<

#-- converting .ps to .pdf.
#%.pdf: %.ps
#	$(PS2PDF) $<

#-- generating pdf using pdflatex
%.pdf: %.tex $(SRCFILES) $(LOCALBIB)
	$(PDFLATEX) $*
#	$(BIBTEX) $*
#	$(PDFLATEX) $*
#	$(BIBTEX) $*
#	$(PDFLATEX) $*
	chmod +x $*.pdf

full: $(SRCFILES) $(LOCALBIB)
	$(PDFLATEX) $(PROJECT)
	$(BIBTEX) $(PROJECT)
	$(PDFLATEX) $(PROJECT)
	$(BIBTEX) $(PROJECT)
	$(PDFLATEX) $(PROJECT)
	chmod +x $(PROJECT).pdf
	

bib:	$(LOCALXTXBIB)
	$(XTEX) --short=state --short=conference --no-field editor --no-field publisher \
		--no-field pages --xtx2bib $(LOCALXTXBIB)

ps:	$(TARGETSPS)

pdf:
	$(PS2PDF) $(TARGETS)

clean:
	rm -f *~  $(TARGETS) $(TARGETSPS) *.dvi *.log *.aux *.blg *.bbl *.out $(OLDAUX)

veryclean: clean
	rm -f $(EPSFIGFILES) $(EPSMFILES) $(EPSPLTFILES)

spell:	$(SRCFILES)
	detex $^ | spell | env LANG=C sort -u | env LANG=C comm -23 - ok-words


==> fig/deadbolt_intersection.tex <==
% \centerline{
\begin{figure}[t]
	\begin{minipage}[t]{0.49\linewidth}
		\centering
		\includegraphics[width=\textwidth]{fig/venn_diagram_btc.png}
		\subcaption{Bitcoin addresses.}
    \label{fig:venn_diagram_btc}
		% Collection includes only samples with at least one AV detection}        
	\end{minipage}
	\hfill
	\begin{minipage}[t]{0.49\linewidth}
		\centering
		\includegraphics[width=\textwidth]{fig/venn_diagram_ips.png}
		\subcaption{IP addresses.}
    \label{fig:venn_diagram_ip}
		\label{fig:2}
	\end{minipage}
	\caption{Overlap in DeadBolt datasets.}
	\label{fig:venn_diagrams}
	\vspace{-0.4cm}
\end{figure}
% }

